Automatic Verification of LLVM Code

In this work we present our work in developing a software verification tool for llvm-code - Lodin - that incorporates both explicit-state model checking, statistical model checking and symbolic state model checking algorithms.

==> symbolic/_region_.tex <==
\message{ !name(symbolic.tex)}
\message{ !name(symbolic.tex) !offset(-2) }
We have already mentioned that an explicit representation of values in
a program will explode (even without concurrency) in the presence of
non-deterministic values. As an example of this, consider
\autoref{lst:symbneed} which can call the function \funcname{@error}
if and only \reg{\%2} is set to $5$. It is easy for easy for humans
to realise that \funcname{@error} can be called, but a computer with an explicit representation has to enumerate
all $32^2-1$ possible values of \reg{\%2}. 
\begin{lstllvm}
  \begin{lstlisting}
    define void @main() #0 {
init:
  %1 = alloca i32, align 4
  %2 = lodin_nd i32
  store i32 %2, i32* %1, align 4
  %3 = load i32, i32* %1, align 4
  %4 = icmp eq i32 %3, 5
  br i1 %4, label %call, label %done

call:                                      ; preds = %0
  call void (...) @error()
  br label %done
  
  done:                                      ; preds = %5, %0
  ret void
}
\end{lstlisting}
\caption{Example of why Symbolic Representation are necessary}\label{lst:symbneed}
\end{lstllvm}

For combatting this, \lodin\ provides a
symbolic context representation. Instead of representing values
explicitly, the symbolic context gathers all operations performed
during exploration into one large logical formula - known as the path
formula -  that can since be passed to
an SMT-solver. The SMT-solver can  then determine if the formula is
satisfiable and thus if the explored path is feasible.

\subsubsection{Satisfiability Modulo Theories }
An SMT-instance is principally a first order logic formula where some
predicates and functions have special interpretations. These special
interpretations are encapsulated into what is called theories. An
SMT-instance of the theory $\theory$ can be determined to be
satisfiable or not satisfiable by SMT-solver supporting the
$\theory$. We will not invest too much time here in talking about how
SMT-solvers work, but will rather informally discuss the theories we need. 

\paragraph{Theory of Bitvectors}
In the theory of bitvectors, variables are given a  bitvector type
\tyi{n}\footnote{Note we reuse the type name from \llvm}.  The operations that can be performed between bitvectors are
\begin{itemize}
\item the classic bitwise operations, i.e. \bitand, \bitor,
  \bitneg, \bitxor, \bitlshl, \bitlshr\ and \bitashr
\item arithmetic operations (modulo $2^n$),
  i.e. \bitadd, \bitsub, \bitudiv, \bitsdiv, \bitmul, \biturem, \bitsrem\ -
  as in the \llvm\ discussion we need both signed and unsigned
  versions of some operations (indexed by $_u$ and $_s$)
\item comparisons e.g. $=$ and $\leq$,
\item boolean  operations \eg ($\wedge, \vee, \lnot$) 
\item concatenation of bitvectors $\bitconcat$,
\item extraction of subvectors i.e. if $\smtvar$ is a bitvector then $b\smtvar[] [0\dots
  n]$ extract a bitvector with bits $0$ to
  $n-1$. 
\end{itemize}

\begin{remark}
  We reuse the operatorions from our discussin of bitvectors in
  \autoref{subsec:expli}, and require that the SMT-solver implements the
  semantics of the operations as described there. Likewise we write constant bitvectors using the notation from \autoref{subsec:expli}.
\end{remark}

\paragraph{Theory of Arrays}
In this theory an array is a mapping between elements. Elements from
an array can be read using  a \arrselect\ function,  and an
element stored in an array using a \arrstore\ function. We introduce
the array type \arrtype{\tyi{n}}{\tyi{m}} mapping elements from
\tyi{n} to \tyi{m}. If $\smtvar \typej \arrtype{\tyi{n}}{\tyi{m}}$,
$\smtvar[1] \typej \tyi{n}$ and $\smtvar[2] \typej \tyi{m}$ then we
write $\arrstore(\smtvar,\smtvar[1],\smtvar[2])$ to create a new array
that is equal to $\smtvar$ with the only difference that the value of
$\smtvar[1]$ now maps to the value of $\smtvar[2]$.  We also write
$\smtvar[2]  = \arrselect(\smtvar,\smtvar[1])$ to set $\smtvar[2]$
equal to the value kept at position $\smtvar[1]$.

In the following we use $\smtvars[]$ to denote an infinite set of SMT
variables. We also use the restricted sets $\smtvars[\ty{ty}] =
\{\smtvar \in\smtvars \mid \smtvar \typej \ty{ty} \}$. Similarly we
refer by $\smtexprs$ to all SMT expressions over $\smtvar$ and
$\smtexprs[\ty{ty}]$ to all SMT expressions with  type $\ty{ty}$.  

3\subsubsection*{The Symbolic Context}
The symbolic context in \lodin\ maps its register variables to SMT
variables and uses a so called path formula to capture all constraints
(assignments and comparisons) encountered during a program
execution. Memory is represented using a SMT array and a SMT variable
points to first place in memory that is free for allocation. 

\newcommand{\used}{\ensuremath{\mathtt{used}}}
\begin{definition}[Symbolic Context]
  The symbolic context for the symbolic semantics is the tuple  $\domainsymbolic = (\domainstates[\domainsymbolic],s_{init},\allowbreak\domainfortypefname{\domainsymbolic},\mathbb{N},\semfalse{\domainsymbolic})$ where
  \begin{itemize}
  \item $\domainstates[\domainsymbolic]$ are tuples
    $(\smtvar[M],\smtvar[f],N,F, \pathform,\used)$ where
    \begin{itemize}
    \item $\smtvar[M] \typej \arrtype{\tyi{64}}{\tyi{8}}$ is an array
      representing the memory state of the program, 
    \item $\smtvar[f] \typej \tyi{64}$ is a pointer into memory 
    \item $N \subseteq \mathbb{N}$ is a set of used register
      variables, 
    \item $ F : \mathbb{N} \rightarrow \smtvars[]\cup\{\bot\}$ 
    \item $\pathform$ is an SMT formula - the path formula - encoding
      the constraints that an explored path has to satisfy, and
    \item $\used\subseteq \smtvars$ is a set of used  SMT variables.
    \end{itemize}
    
  \item $s_{init} = (M,0,F,\semfalse{\domainsymbolic} == \semfalse{\domainsymbolic},\emptyset)$ where for all $n\in\mathbb{N}$ , $F(n) = \bot$
  \item $\domainfortypefname{\domainsymbolic}(\tyi{i}) =
    \smtvars[\tyi{i}]$, $\domainfortypefname{\domainsymbolic}(\ptr{ty}) = \smtvars[\tyi{64}]$, and  
    $\domainfortypefname{\domainsymbolic}(\comptype{\ty{ty1},\dots\ty{ty1n}}) = \smtvars[8\cdot\bytesize(\comptype{\ty{ty1},\dots\ty{ty1n}})]$
  \item $\semfalse{\domainsymbolic} = \zerovec{8}$. 
  \end{itemize}
\end{definition}

The arithmetic instructions (e.g. $\semadd{\ty{ty}}{\domainsymbolic}(\domainstate, \smtvar[1],\smtvar[2]$) that we need to implement for the context is
straightforward to represent. All we need to do is to create an SMT expressions corresponding to the operation,
 Below we give a generalised definition of the rule:

\begin{align*}
  \sim^{\ty{ty}}_{\domainsymbolic} &((\smtvar[M],\smtvar[f],F,
                   \pathform,\used),\smtvar[1],\smtvar[2]) = \smtvar[1]\,\mathtt{SMTOp}\, \smtvar[2]\\
\end{align*}
 For the mapping between $\sim^{\ty{ty}}_{\domainsymbolic}$  and
$\mathtt{SMTOp}$ we 
refer to \autoref{tab:opsmtop}.

The comparison operators are very similar to the binary operator, and
below we provide an example for the
$\semugt{\ty{ty}}{\domainsymbolic}(\domainstate,\smtvar[1],\smtvar[2])$ function
where $\domainstate =  (\smtvar[M],\smtvar[f],F, \pathform,\used)$

\begin{align*}
  \semugt{\ty{ty}}{\domainsymbolic}(\domainstate,\smtvar[1],\smtvar[2])
  = &(\smtvar[M],\smtvar[f],N,F, \pathform\wedge (\smtvar[3] =
                                                   (\smtvar[1] >_u
                                                   \smtvar[2]), \\
                                                 &\used\cup\{\smtvar[3]),\smtvar[3],\top)
\end{align*}

For the remainder of the operations we
refer the reader to \autoref{fig:evalsetsymb} and \autoref{fig:loadstoresymb}.
\renewcommand{\arraystretch}{1.5}
\begin{table}[t]
  \centering
  \begin{tabular}{|l|l|}
    \semadd{\ty{ty}}{\domainsymbolic} & \bitadd \\
    \semsub{\ty{ty}}{\domainsymbolic} & \bitsub \\
    \semmul{\ty{ty}}{\domainsymbolic} & \bitmul \\
    \semudiv{\ty{ty}}{\domainsymbolic} & \bitudiv\\
  \end{tabular}\hfill
  \begin{tabular}{|l|l|}
    \semsdiv{\ty{ty}}{\domainsymbolic} & \bitsdiv \\
    \semurem{\ty{ty}}{\domainsymbolic} & \biturem\\
    \semsrem{\ty{ty}}{\domainsymbolic} & \bitsrem\\
    \semshl{\ty{ty}}{\domainsymbolic} & \bitlshl\\
  \end{tabular}\hfill
  \begin{tabular}{|l|l|}
    \semlshr{\ty{ty}}{\domainsymbolic} & \bitlshr\\
    \semashr{\ty{ty}}{\domainsymbolic} & \bitashr\\
    \semand{\ty{ty}}{\domainsymbolic} & \bitand\\
    \semor{\ty{ty}}{\domainsymbolic} & \bitor\\
    \semxor{\ty{ty}}{\domainsymbolic} & \bitxor\\
  \end{tabular}
  \caption{Mapping between semantical operators and SMT operators\label{tab:opsmtop}}
\end{table}


\begin{figure*}
  \centering
  \begin{mathpar}
    \semmakereg{\domainsymbolic}((\smtvar[M],\smtvar[f],N,F,\pathform,\used),\reg{\%r})
    = (\smtvar[M],\smtvar[f],N\cup\{i\},F,\pathform,\used),i \text {
      where } i = \dmin (\mathbb{N}\setminus N) \and

    \semevalreg{\domainsymbolic}((\smtvar[M],\smtvar[f],N,F,\pathform,\used),i)
    =
    \begin{cases}
      F(i) & \text{ if } F(i) \in \domainfortype[\domainsymbolic]{\ty{ty}}\\
      \mathbf{Error} & \text { Otherwise } \\
    \end{cases} \and
    \semset{\ty{ty}}{\domainsymbolic}((\smtvar[M],\smtvar[f],N,F,\pathform,\used),l,\smtvar)
    = \begin{cases}
      (\smtvar[M],\smtvar[f],N,F,\pathform\wedge (F(l) = \smtvar),\used) & \text{ if } l\in N \land \smtvar\in\domainfortypefname{\domainsymbolic}(\ty{ty})\\
      \mathbf{Error} & \text { Otherwise } \\
    \end{cases} \and
    \semalloc{\ty{ty}}{\domainsymbolic}((\smtvar[M],\smtvar[f],N,F,\pathform,\used))
    =
    \begin{cases}
      (\smtvar[M],\smtvar[f'],N,F,\pathform\wedge (\smtvar[f']=\smtvar[f]\bitadd n),\used\setminus\{\smtvar[f]\}),\smtvar[f]& \text{ if } \ty{ty} = \tyi{n}     \\
      (\smtvar[M],\smtvar[f'],N,F,\pathform \wedge (\smtvar[f']=\smtvar[f]\bitadd 64),\used\setminus\{\smtvar[f]\}),\smtvar[f] & \text{ if } \ty{ty} = \ptr{\tyi{n}} \\
    \end{cases} \and
    \semptradd[\domainsymbolic](\smtvar[b_1],k) = \smtvar[b_1] \bitadd k

  \end{mathpar}
  
  \caption{Evaluation and setting registers in symbolic context.}
  \label{fig:evalsetsymb}
\end{figure*}


\newcommand{\loadinner}[1]{\ensuremath{\mathtt{SymbLoad}^{#1}}}
\newcommand{\storeinner}[1]{\ensuremath{\mathtt{SymbStore}^{#1}}}

\begin{figure*}[t]
  \centering
  \begin{mathpar}
    \semload{\tyi{n}}{\domainsymbolic}((\smtvar[M],\smtvar[f],N,F,\pathform,\used),i)
    = \loadinner{\tyi{n}}(\smtvar[M],F(i)) \\ \and
    \loadinner{\tyi{n}}(\smtvar[M],\smtvar[a]) =
    \begin{cases}
      \arrselect (\smtvar[M],\smtvar[a])& \text{ if } \tyi{n} =
      \tyi{8}
      \\
      \arrselect (\smtvar[M],\smtvar[a])\bitconcat
      \loadinner{\tyi{n-8}}(\smtvar[M],\smtvar[a]\bitadd 1 ) & \text{
        otherwise}
    \end{cases}
  
    \semstore{\ty{ty}}{\domainsymbolic}((\smtvar[M],\smtvar[f],N,F,\pathform,\used),\smtvar[v],\smtvar[p])
    = (\smtvar[M'],\smtvar[f],N,F,\pathform\wedge (\smtvar[M'] =
    \storeinner{\ty{ty}} (\smtvar[M],\smtvar[v],\smtvar[p]))
    ,\used,\smtvar[v],\smtvar[p])

    \storeinner{\tyi{n}} ((\smtvar[M],\smtvar[v],\smtvar[p])) =
    \begin{cases}
      \arrstore(\smtvar[M],\smtvar[p],\smtvar[v]) & \text{ if }
      \tyi{n} =
      \tyi{8} \\
      \storeinner{\tyi{n-8}}
      (\arrstore(\smtvar[M],\smtvar[p],\smtvar[v][0\dots
      8]),\smtvar[p]\bitadd 1, \smtvar[v][8\dots n ])& \text{ otherwise
      }
    \end{cases}

  \end{mathpar}
  
  \caption{Store and Load operations in the symbolic context}
  \label{fig:loadstoresymb}
\end{figure*}

\begin{example}
  We briefly return to the module ($\module$) in \autoref{lst:symbneed} and consider how
  we can use the symbolic representation of \lodin\ to determine if
  the function \funcname{error} can be called. We simply
  instantiate the symbolic transition system $\lts{\domainsymbolic}{\module} =
(\netstates[\domainsymbolic],\netinitstate[\domainsymbolic],\systranssymb{})$
and generate symbolic states from $\netinitstate[\domainsymbolic]$ until we reach a state $\netstate[f] =
(s_1:s_2\dots:\emptylist,\domainstate[\domainsymbolic],\module)$ where $s_1 =
(\funcname{main},\lllabel{prev},\lllabel{call},\pc,\registermap,\frees)$
and $\domainstate[\domainsymbolic] = (\smtvar[M],\smtvar[f],N,F,
\pathform,\used)$.  Reaching $\netstate[f]$ reveals that there is a path in the control
flow graph of $\funcname{main}$ that reaches the call-block (and
thereby the call instruction), but not that it is feasible. To ensure
the feasibility, we invoke a SMT-solver and checks if
$\pathform$ is satisfiable. If this is the case, we can read the value
of all registers used along that path from the SMT satisyfing
assignment. 
\end{example}

\paragraph{Merging Symbolic States}
\newcommand{\mergef}{\ensuremath{\mathtt{merge}}}
It is usual convenient to merge symbolic context states into one
state. This allows exploring several computational paths simultaneously and
helps combat path-explosion problem - which  is a big problem for
symbolic execution engines such as \klee.

For merging context-states \[\domainstate[\domainsymbolic] = 
(\smtvar[M],\smtvar[f],N,F, \pathform,\used)\] and
\[\domainstate[\domainsymbolic]' = (\smtvar[M]',\smtvar[f]',N',F',
\pathform',\used')\] where for all $n\in N\cap N'$ it is the case that $F(n) =
F'(n)$  we introduce the function $\mergef :
\domainstates[\domainsymbolic]\times
\domainstates[\domainsymbolic]\rightarrow
\domainstates[\domainsymbolic]$ defined as

\begin{align*}
\mergef(\domainstate[\domainsymbolic],&\domainstate[\domainsymbolic]')
= (\smtvar[M]'',\smtvar[f]'',N\cup N',F'',(\pathform\vee\pathform') \wedge
\pathform''\wedge \pathform''',\\
&\used\cup\used'\cup\{\smtvar[M]'',\smtvar[f]'',\smtvar[P]\})
\end{align*}
where  
\begin{itemize}
\item $F''(n) =
  \begin{dcases}
    F(n) & \text{ if } n\in N\\
    F'(n) & \text{ if } n\in N'\\
  \end{dcases}$
\item $\smtvar[M]'',\smtvar[f]'',\smtvar[P]\notin\used\cup\used'$,
\item $\syntaxeq{\pathform''}{\smtvar[M]'' = \smtite{\smtvar[P]}{\smtvar[M]}{\smtvar[M']}}$,
\item $\syntaxeq{\pathform'''}{\smtvar[f]'' = \smtite{\smtvar[P]}{\smtvar[f]}{\smtvar[f']}}$. 
\end{itemize}

Here $\smtvar[P]$ with type $\tyi{8}$ is a fresh SMT variable and
$\smtite{\smtvar[P]}{\smtvar}{\smtvar'}$ evaluates to $\smtvar'$ if
  $\smtvar[P] = \semfalse{\domainsymbolic}$ and to $\smtvar$ otherwise.
\message{ !name(symbolic.tex) !offset(-307) }

